Link Prediction using Embedded Knowledge Graphs

Since large knowledge bases are typically incomplete, missing facts need to be inferred from observed facts in a task called knowledge base completion. The most successful approaches to this task have typically explored explicit paths through sequences of triples. These approaches have usually resorted to human-designed sampling procedures, since large knowledge graphs produce prohibitively large numbers of possible paths, most of which are uninformative. As an alternative approach, we propose performing a single, short sequence of interactive lookup operations on an embedded knowledge graph which has been trained through end-to-end backpropagation to be an optimized and compressed version of the initial knowledge base. Our proposed model, called Embedded Knowledge Graph Network (EKGN), achieves new state-of-the-art results on popular knowledge base completion benchmarks.

==> apply_to_kbc.tex <==
\section{Applying \generalmodelname/ to Knowledge Base Completion}
\label{sec:kbc}

%We also missing a lot of details in the KBC part
The goal of KBC tasks \citep{BUGWY13} is to predict a head or a tail entity given the relation type and the other entity, i.e. predicting $h$ given $(?,r,t)$ or predicting $t$ given $(h, r, ?)$, where $?$ denotes the missing entity. %For each testing triple, the head or tail is removed and replaced by each of the entities of the dictionary in turn. Dissimilarity (or distance) function of those corrupted triples are computed by the models and then sorted by ascending order.
% describe input/output
%% input
For a KBC task, the input to our model is a subject entity (a head or tail entity) and a relation. The task-dependent input module first extracts the embedding vectors for the entity and relation from an embedding matrix. We then represent the query vector $q$ for an \modelname/ as the concatenation of the two vectors.
% global memory
We randomly initialize the global memory component. At each step, a training triple is processed through the model by Algorithm \ref{alg:inference_process}, where no explicit path information is given. 
The \modelname/ updates the global memory implicitly with respect to the objective function.
%% output
For the task dependent output module, we use a nonlinear projection to project the controller state into an output vector $o$: $f_o(s_t; \theta_o) = \text{tanh}({W_o} s_t + {b_o})$, where the $W_o$ and $b_o$ are the weight matrix and bias vector, respectively. 
We define the ground truth target (object) entity embedding as $y$, and use the $L_1$ distance measure between the output $o$ and target entity $y$, namely $d(o, y) =| o-y |_1$. 
We sample a set of incorrect entity embeddings $N = \{y^-_i\}_{i=1}^{|N|}$ as negative examples. The probability of selecting a prediction $\hat{y} \in D$ can be approximated as 
\[ \label{softmax_sample}
p(\hat{y}|o) = \frac{\exp(-\gamma d(o,\hat{y}))}{\sum_{y_k \in {D}} \exp(-\gamma d(o, y_k)) }
\]
where $D = N \cup \{y\}$. We set $|N|$ and $\gamma$ to 20 and 5, respectively, for the experiments on FB15k and WN18 datasets.
The \modelname/ performs a prediction action $p_T$ on selecting $\hat{y}$ with probability $p(\hat{y}|o)$ . We define the reward of the prediction action as one if the ground truth entity is selected, and zero otherwise. 

%
%
%TransE \cite{BUGWY13} is a typical knowledge base embedding method for KBC task. It learns vectors (i.e., embeddings) for both entities and relations from a set of training triples. However, TransE and its variant models  only reply on learning ideal relation embeddings to help with the KBC task. We propose \modelname/ model that can execute multiple step inference over a global memory to search for missing tail entity given the head entity and relation type. 
%
%Following the neural-based KBC approaches, consider each entity in knowledge based is encoded with two vectors : $e^{in}$ and $e^{out}$; and each relation type encoded with one vector $r$. Give the head entity and relation type, the input module of \modelname/ concatenate $e_{head}^{in}$ and $r$ to obtain the input representation, $q=[e_{head}^{in}; r]$, the output module of \modelname/ aims to produce a output vector to approximate the out embedding of the missing tail entity, $a = e_{tail}^{out}$ \footnote{In literature, some of embedding models, i.e., TransE \cite{BUGWY13}, tie $e^{in}$ and $e^{out}$ together. }.



% We apply a nonlinear projection as the output module: $f_o(s_t; \theta_o) = \text{tanh}(\mathbf{w_o} s_t + {b_o})$; $\theta_o = (\mathbf{w_o}, {b_o})$

% setup
%We use the same hyper-parameters for both FB15k and WN18 data sets. Entity embeddings (Input and Output) and relation embedding are both 100-dimensions. There are 64 memory vectors with 200 dimensions each, initialized by random vectors with unit L2-norm. We apply a GRU with 200 cells as the controller. We choose projected cosine similarity function as the attention module. The attention score $a_{t,i}$ on memory $m_i$ given state $s_t$ is computed as $a_{t,i} = \text{softmax}_{i=1,...,|M|} \lambda \cos(\mathbf{w_1} m_i, \mathbf{w_2} s_t)$ \footnote{$\lambda$ is set to 10 in experiments.}. Attention vector $x_t$ is thus, given by $x_t = \sum_{i}^{|M|} a_{t,i} m_i$. The termination variable is modeled by a logistical regression approach : $f_t(s_t; \theta_t) = \text{sigmoid}(\mathbf{w_t} s_t + {b_t})$; $\theta_t = (\mathbf{w_t}, {b_t})$. We apply a nonlinear projection as the output module: $f_o(s_t; \theta_o) = \text{tanh}(\mathbf{w_o} s_t + {b_o})$; $\theta_o = (\mathbf{w_o}, {b_o})$ .

%
% We set the maximum number of reasoning steps of \modelname/ to 5. We randomly initialize all model parameters, and use SGD as the training algorithm with mini-batch size of 64. We set the learning rate to a constant number, 0.01. To prevent the model from learning a trivial solution by increasing entity embeddings norms, we follow the work in \cite{BUGWY13} to enforce the $L_2$-norm of the entity embeddings as 1.
%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> model.tex <==





% rewrite after intro.
% motivation of model design
% a. Intuition: why such design can solve compositionality implicitly: explain why memory: why attention

% b. Explain why multiple steps (compositionality)
\begin{figure*}[t!]
	\quad\quad\quad\quad
	{\tiny }	\includegraphics[width=0.78\textwidth]{figures/architecture.pdf} % use pdf
	\caption{An \modelname/ Architecture.}
	\label{fig:implicit_reasonet}
\end{figure*}

% Introduction
%Say we will induce a general model first and then adapt to the KB later
% In this section, we introduce our proposed \modelname/ model in
% Section \ref{sec:architecture}. % The training algorithm detailed
% setting to KBC tasks in Section \ref{sec:training_objective}.

% a. The components
In this section, we describe the general architecture of \generalmodelname/ in a way that is agnostic to KBC.
\generalmodelname/ are composed of four main components: an input
component, an output component, a global memory, and a search
controller, as shown in Figure \ref{fig:implicit_reasonet}. In this section, we briefly describe each component.
% i. What is input component

\underline{Input/Output Modules}: These two modules are task-dependent. The input module takes a query and converts the query into a
vector representation $q$. The output module is a function $f_o$, 
which converts the hidden state received from the search controller
($s$) into an output $O$. We optimize the whole model using the
output prediction $O$ with respect to a ground-truth target using a
task-specified loss function.

%iii. What is the global memory (say it will be be clear)
\underline{Global Memory}: The global memory is denoted as $M$. It
consists of a list of memory vectors, $M = \{m_i \}_{i=1...I}$, where
$m_i$ is a fixed dimensional vector. The memory vectors are randomly
initialized and automatically updated through back-propagation. The
global memory component is shared across all instances.

%iv. Search controller
\underline{Search Controller}: The search controller is a recurrent
neural network and controls the search process by keeping internal
state sequences to track the current search process and history. The search controller uses an attention mechanism to fetch information from relevant memory vectors in $M$, and decides if the model should output the prediction
or continue to generate the next possible output.

\begin{itemize}
	\item \textit{Internal State}: The internal state of the search controller is denoted as $S$, which is a vector representation of the search process. The initial state $s_1$ is usually the vector representation of the input vector $q$. The internal state at $t$-th time step is represented by $s_t$. The sequence of internal states is modeled by an RNN: $s_{t+1} = \text{RNN}(s_t, x_t; \theta_s)$.
	
	\item \textit{Attention to memory}: The attention vector $x_t$ at $t$-th time step is generated based on the current internal state $s_t$ and the global memory $M$: $x_t = f_{att}(s_t, M; \theta_x)$.
	Specifically, the attention score $a_{t,i}$ on a memory vector $m_i$ given a state $s_t$ is computed as $a_{t,i} = \text{softmax}_{i=1,...,|M|} \lambda \cos({W_1} m_i, {W_2} s_t)$, where $\lambda$ is set to 10 in our experiments and the weight matrices ${W_1}$ and ${W_2}$ are learned during training. The attention vector $x_t$ can be written as $x_t = f_{att}(s_t, M; \theta_x)=  \sum_{i}^{|M|} a_{t,i} m_i$. 
	
	\item \textit{Termination Control}: The terminate gate produces a stochastic random variable according to the current internal state, $t_t \sim p( \cdot |f_{tc}(s_t; \theta_{tc})))$. $t_t$ is a binary random variable. If $t_t$ is true, the \modelname/ will finish the search process, and the output module will execute at time step $t$; otherwise the \modelname/ will generate the next attention vector $x_{t+1}$ and feed into the state network to update the next internal state $s_{t+1}$.	
	In our experiments, the termination variable is modeled by a logistical regression: $f_{tc}(s_t; \theta_{tc}) = \text{sigmoid}({W_{tc}} s_t + {b_{tc}})$, where the weight matrix ${W_{tc}}$ and bias vector $b_{tc}$ are learned during training.
\end{itemize}

 Compared \generalmodelname/ to Memory Networks (MemNN)~\citep{WestonChBo14,key_value_memnn_emnlp16} and Neural Turing Machines (NTM) \citep{GravesWaDa14,
  GWRHDGCGRAo16}, the biggest difference between our model and the
existing frameworks is the search controller and the use of the shared
memory.  
We follow \citet{Reasonet16} for using a
%We build upon our previous work \citep{Reasonet16} for using a
search controller module to dynamically perform a
multi-step inference depending on the complexity of the instance.
%The search controller allows us to dynamically perform a multi-step inference depending on the complexity of the instance.
% problem: compare to MemNN - they have global memory as well (key-value MemNN)
MemNN and NTM explicitly store inputs (such as graph definition, supporting facts) in the memory. In contrast, in \generalmodelname/, we do not explicitly store all the observed inputs in the global memory. Instead, we directly operate on the global memory, which modeling the structured relationships implicitly. We randomly initialize the memory and update the memory with respect to task-specific objectives.
% problem: compare to neural semantic encoder - different purpose, differnet operation
The idea of exploiting global memory is proposed
by~\citet{MunkhdalaiY16} independently.  Despite of using the same
term, the goal and the operations used by \generalmodelname/ are
different from the one used in~\citet{MunkhdalaiY16}, as
\generalmodelname/ allow the model to perform multi-step for each
instance dynamically.

\ignore{ % fore rebuttal
  In~\citet{MunkhdalaiY16,162}, the input instance encoding and the memory
  access is synchronized, as the number of memory access is equal to
  the input length. In our work, the number of memory access is decided by the
  complexity of instance, which is modeled by the search controller.

  %The work you have mentioned is very close to our earlier work
  %\citep{Reasonet16} that we built upon. It would be interesting if
  %you can clarify the differences on discussion area the corresponding
  %submission.
  }

  \subsection{Stochastic Inference Process}
%b. How everything work together
%Explain algorithm 1 in detail
%Why is this similar to search?
The inference process of an \modelname/ is as follows. First, the model
converts a task-dependent input to a vector representation through
the input module. Then, the model uses the input representation to
initialize the search controller. In every time step, the search
controller determines whether the process is finished by sampling
from the distribution according to
the terminate gate. If the outcome is termination, the output module will generate a
task-dependent prediction given the search controller states. If the outcome
is continuation, the search controller will move on to the next time step,
and create an attention vector based on the current search controller
state and the global memory.  Intuitively, we design
whole process by mimicking a search procedure that iteratively finds
its target through a structure and output its prediction when a
satisfying answer is found.  The detailed inference process is
described in Algorithm \ref{alg:inference_process}.
%we describe the process of generating output vector in \modelname/ given the input query vector.
 
 \begin{algorithm}[t]
 	\SetKwInOut{Input}{Input}
 	\SetKwInOut{Output}{Output}
 	\Input{Randomly initialized global memory $M$; Input vector $q$; Maximum step $T_{\text{max}}$}
 	\Output{Output vector $o$}
 	Define $s_1 = q$; $t = 1$\;
 	Sample $t_t$ from the distribution $p(\cdot|f_{tc}(s_t; \theta_{tc}))$\;
 	if $t_t$ is false, go to Step 4; otherwise Step 7\;
 	Generate an attention vector $x_t = f_{att}(s_t, M; \theta_{x})$\;
 	Update the internal state $s_{t+1} = \text{RNN}(s_t, x_t; \theta_s)$\;
 	Set $t = t + 1$; if $t < T_{\text{max}}$ go to Step 2; otherwise Step 7\;
 	Generate output $o_t = f_o(s_t; \theta_o) $\;
 	Return $o = o_t$\;
 	\caption{Stochastic Inference Process in an \modelname/}
 	\label{alg:inference_process}
 \end{algorithm}

%\subsection{Property of \generalmodelname/}


%\modelname also focuses on different types of tasks compared to
%~\citep{GravesWaDa14, GWRHDGCGRAo16, Reasonet16}.

% In contrast, \modelname/ tackles the problems of {\em implicit
%   structures search}, where the structure of the task $G$ is not
% explicitly given. Models need to perform search based on the partially
% observed information, namely the pair of $q$ and $a$ from the training
% data.  This can be explained on the synthetic tasks have started
% evaluating the inference ability of the neural models using various
% synthetic tasks. One popular type of synthetic tasks are what we
% called {\em explicit structures search}. In the explicit structures
% search task, an input instance is a tuple $(G,q)$, where $G$
% represents the structure of the task and $q$ represents the query. The
% output of the example is $a$, which represents the answer of the
% query. The task expects the model to perform search within the scope
% of $G$. For example, in the differentiable neural computer work
% \citep{GWRHDGCGRAo16}, one of the tasks is to find a shortest path
% between two nodes ($q$) in the given graph ($G$). The answer ($a$) of
% example should be one of the shortest path between the nodes.
% However, search over explicit structures tasks only operates on small
% scale problems with a clearly defined structure (e.g. graph), limiting
% the their usage of measuring the usefulness of neural models on real
% tasks.

%
%c. Compare to other framework
%
\subsection{Motivating Example of Operation}
% how it work
We now describe an example of how our model can perform inference on-the-fly as it is reading input instances. 
Suppose, in a knowledge base completion task, the input is (\texttt{Obama}, \textsc{Nationality}, ?) and the model is required to answer the missing entity (answer: \texttt{U.S.A}).
Our model can learn to utilize and store information in the global memory through the search controller. 
% new information
When a new information from a new instance is received (e.g., (\texttt{Obama}, \textsc{BornIn}, \texttt{Hawaii})), the model first uses its search controller to find relevant information. If the relevant information is not found, the model learns to store the information to memory vectors by gradient update in order to answer the missing entity correctly. 
% Old information
Due to the limited size of the global memory, the model cannot learn to store all new information explicitly. 
The model needs to learn to utilize the global memory efficiently to lower the training loss. 
If a related information from a new instance is received (e.g., (\texttt{Hawaii}, \textsc{PartOf}, \texttt{U.S.A}), the model learns to do inference by utilizing the search controller to go over existing memory vectors iteratively. 
In this way, the model could learn to do inference and correlate training instances via memory cells without explicitly storing a new information.
For semantically relevant relations, such as \textsc{Nationality} and \textsc{BornIn}, the model could learn to correlate them and compactly represent them using similar representations in the memory cells. 


\ignore{
A knowledge base usually has a graph structure which consists of a set of  triples of the form $(e_{head}, r, e_{tail})$ where $e_{head}, e_{tail} \in {E}$ and $r \in {R}$. Let $E$ be the set of entities and $R$ be the set of relations. Knowledge base completion is the task of predicting missing tail entity given the head entity and relation type.

TransE \citep{BUGWY13} is a typical knowledge base embedding method for KBC task. It learns vectors (i.e., embeddings) for both entities and relations from a set of training triplets. However, TransE and its variant models  only reply on learning ideal relation embeddings to help with the KBC task. We propose \modelname/ model that can execute multiple step inference over a global memory to search for missing tail entity given the head entity and relation type. 

Following the neural-based KBC approaches, consider each entity in knowledge based is encoded with two vectors : $e^{in}$ and $e^{out}$; and each relation type encoded with one vector $r$. Give the head entity and relation type, the input module of \modelname/ concatenate $e_{head}^{in}$ and $r$ to obtain the input representation, $q=[e_{head}^{in}; r]$, the output module of \modelname/ aims to produce a output vector to approximate the out embedding of the missing tail entity, $a = e_{tail}^{out}$ \footnote{In literature, some of embedding models, i.e., TransE \citep{BUGWY13}, tie $e^{in}$ and $e^{out}$ together. }.
    

\textbf{Internal State}: The internal state is denoted as $S$ which is a vector representation of the input state. The initial state $s_1$ is usually the vector representation of the input question. The $t$-th time step of the internal state is represented by $s_t$. The sequence of internal states is modeled by an RNN: $s_{t+1} = \text{RNN}(s_t, x_t; \theta_s)$.

\textbf{Global Memory}: The global memory is denoted as $M$. It consists of a list of memory vectors, $M = \{m_i \}_{i=1...D}$, where $m_i$ is a fixed dimensional vector. The memory vectors are randomly initialized and automatically updated through back-propagation. The global memory component is shared across all of the instances.

\textbf{Attention}: The attention vector $x_t$ at $t$-th time step is generated based on the current internal state $s_t$ and the global memory $M$: $x_t = f_{att}(s_t, M; \theta_x)$;



% why a dot there???
\textbf{Termination Gate}: The termination gate produces a stochastic random variable according to the current internal state, $t_t \sim p( \cdot |f_t(s_t; \theta_t)))$. $t_t$ is a binary random variable. If $t_t$ is true, the \modelname/ will stop, and the answer module will execute at time step $t$; otherwise the \modelname/ will generate the next attention vector $x_{t+1}$, and feed into the state network to update the next internal state $s_{t+1}$.

\textbf{Output}: The output module will be triggered when the termination gate variable is true: $o_t = f_o(s_t ; \theta_o) $. 
}

%We propose \modelname/ to address the compositionality problem. \modelname/ is coupled with a global memory module to implicitly store structured information among instances and uses the attention mechanism to only focus on relevant memory cells given an input state. Because of different levels of difficulty among instances, some instances might require to be decomposed into multiple segments. \modelname/ utilizes an RNN controller to repeatedly read the implicit memory module with attention until a satisfied answer is found.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

